Precision QCD at the LHC: from the structure of the proton to all-order resummations

Experiments at the LHC are collecting a wealth of data with an unprecedented level of precision. As a consequence, the theoretical error is now starting to lag behind the experimental one, and a ceaseless effort is required to reduce the theory uncertainty to match the precision of the data. At hadron colliders, QCD predictions are obtained by convoluting perturbative parton-level results with non-perturbative PDFs, whose precise determination is crucial to reach percent-accurate theoretical predictions. At the parton level, cross sections are obtained through a perturbative expansion in the strong coupling. In some cases, large terms appear at all orders and spoil the convergence of the series. The perturbative description is rescued by resumming the series to all orders, thereby making theory calculations accurate in regions where a fixed-order treatment is not sufficient. In this thesis I first present two global PDF sets where fixed-order calculations are supplemented by threshold and high-energy resummation, respectively. In the first case, it is found that including resummation into PDFs can compensate for the enhancement in the partonic cross sections, with implications for high-mass resonance searches. In the second case, resummation quantitatively improves the description of the HERA structure functions, thus providing evidence of the onset of a new dynamical regime of QCD in the HERA data. I then focus on Higgs production in gluon fusion. The effect of threshold resummation on the total cross section is found to significantly improve the convergence of the perturbative series and to provide a robust method for estimating missing higher order uncertainty. Finally, I present predictions for the Higgs transverse-momentum spectrum both in the inclusive case and within fiducial cuts, exploiting a novel approach where transverse-momentum resummation is performed in direct space.

==> chapters/app1-pdf.tex <==
\begin{savequote}[8cm]
\textlatin{With four parameters I can fit an elephant, and with five I can make him wiggle his trunk.}

  \qauthor{--- Johnny von Neumann}
\end{savequote}

\chapter{\label{ch-pdf}Parton Distribution Functions \amper their determination} 

%\minitoc

Parton Distribution Functions are a central ingredient for theoretical predictions within the QCD factorization framework. 
%
Unlike the strong coupling, PDFs are not fundamental quantities; nevertheless, currently they cannot be determined from first principles and need to be extracted from fits to experimental data.
%
Like the strong coupling, however, parton densities obey a renormalization group equation, the Dokshitzer-Gribov-Lipatov-Altarelli-Parisi (DGLAP) equation~\cite{Gribov:1972ri,Lipatov:1974qm,Altarelli:1977zs,Dokshitzer:1977sg}, which perturbatively controls their dependence on the factorization scale $\mu_F$. 


The accurate knowledge of PDFs is a primary component in the physics precision programme at the Large Hadron Collider.
%
PDF uncertainties affect several probes at the LHC; for instance, they are among the dominant sources of uncertainties in Higgs coupling measurements~\cite{deFlorian:2016spz}, as well as in precise measurement of the strong coupling constants~\cite{Khachatryan:2014waa,Chatrchyan:2013txa,Bouzid:2017uak,Aaboud:2017fml,Klijnsma:2017eqp,Andreev:2017vxu, Johnson:2017ttl,Britzger:2017maj}, or in the extraction of the $W$ mass~\cite{Bozzi:2011ww,Bozzi:2015hha,Bozzi:2015zja,Aaboud:2017svj}.
%
Due to poor constraint at large $x$, PDFs uncertainties are also a primary source of uncertainty in the production of high-mass Beyond Standard Model (BSM) resonances. 
%
Besides collider physics, the precision to which PDFs are known plays a role also in other cases, \emph{e.g.} in astrophysical processes with ultra-high energy neutrinos~\cite{CooperSarkar:2011pa,Gauld:2015kvh,Garzelli:2016xmx}.

Updated PDF sets are regularly being released by various collaborations.
%
These sets are determined using data from a variety of high-energy scattering processes in lepton-hadron and in hadron-hadron collisions. 
%
The analyses differ in several aspects, such as the input dataset used, methodology, error estimate, as well as theoretical differences in the computations of the cross-sections and in the treatment of heavy quarks. 

In this Chapter we will describe some aspects of PDFs and their determination.
%
We will start by discussing the scale dependence and some general features of parton distributions.
%
We will then analyse in some detail the treatment of heavy quarks, focusing in particular on the role of the charm quark.
%
Finally, we will review the fitting procedures used by different collaborations and we will describe their methodology. 
%
 
\section{Scale dependence of Parton Distribution Functions}

The value of parton densities $f(x,\mu_F^2)$ at a fixed scale $\mu_F$ and their dependence on the momentum fraction $x$ are not calculable in perturbation theory.
%
However, the scale dependence of PDFs is computable in perturbative QCD.
%
A rigorous proof of the PDF scale dependence can be obtained by using the operator product expansion (OPE) formalism; here we will present a simplified derivation based on the factorization scale independence of the physical cross sections.

\subsection{DGLAP evolution}

Let us start by considering the factorization scale dependence of structure functions in DIS. 
%
For simplicity, let us assume that there is only one species of quarks in the target, and thus the structure function can be written as eq.~\eqref{eq:structfuncMSbar}.
%
By imposing that the structure function is independent of the factorization scale,
\begin{equation}
	\mu_F^2 \frac{\partial}{\partial \mu_F^2} F (x, \mu_F^2) = 0
\end{equation}
we obtain the following renormalization group equations (RGE) for the parton densities:
\begin{equation}\label{eq:simpleDGLAP}
	\mu^2 \frac{\partial}{\partial \mu^2} q(x,\mu^2) =\frac{\as(\mu^2)}{2 \pi}  \int_x^1 \frac{dz}{z} P\left( \frac{x}{z} \right) q(z,\mu^2) 
\end{equation}
where we dropped the subscript $F$ for readability. 
Note that the coupling is evaluated at $\mu^2$, thus by solving eq.~\eqref{eq:simpleDGLAP} all the leading-log terms $\as^n (\mu^2) \ln^n \mu^2$ are resummed.
%
In the case of deep-inelastic scattering collisions, this result can be proven at all orders in perturbation theory using a rigorous treatment based on the renormalization group equation and OPE~\cite{Georgi:1951sr,Gross:1974cs}.


In this simplified derivation we have considered only the possibility that quarks radiate gluons.
%
However, we have to take into account also the presence of gluons in the target hadron, as the quark struck by the electroweak boson can be produced by gluon splitting.
%
Moreover, we have to include quarks of different flavours.
%
The evolution equation~\eqref{eq:simpleDGLAP} thus takes the general form
\begin{equation}\label{eq:AP}
		\mu^2 \frac{\partial}{\partial \mu^2} f_i(x,\mu^2) =\int_x^1 \frac{dz}{z} P_{ij}\left(\frac{x}{z},  \as(\mu^2) \right) f_j(z,\mu^2), 
\end{equation}
which is the renowned DGLAP equation~\cite{Gribov:1972ri,Lipatov:1974qm,Altarelli:1977zs,Dokshitzer:1977sg}.
%
In eq.~\eqref{eq:AP}, $P_{ij} (z, \as)$ is a $(2n_f +1) \times (2n_f +1)$ matrix of Altarelli-Parisi splitting functions, which can be espanded in powers of the strong coupling as
\begin{equation}
	P_{ij} (z, \as) = \as \left[ P^{(0)}_{ij} (z) +  \as P^{(1)}_{ij} (z) +  \as^2 P^{(2)}_{ij} (z) + \mathcal O(\as^3) \right].
\end{equation}
The coefficients $P^{(k)}_{ij}$ can be calculated in perturbation theory, and are currently known at NNLO accuracy~\cite{Moch:2004pa,Vogt:2004mw}. 
%
%The LO~\cite{Altarelli:1977zs} and NLO~\cite{Curci:1980uw,Furmanski:1980cm,Floratos:1977au,Floratos:1978ny,GonzalezArroyo:1979df,Floratos:1981hs} splitting functions were known since a long time, whereas it took quite some time to obtain the NNLO ones~\cite{Moch:2004pa,Vogt:2004mw}.
%%
%First results towards the N$^3$LO splitting functions have been presented recently~\cite{Ablinger:2017tan,Moch:2017uml}.
%
Due to charge conjugation and $SU(n_f)$ flavour symmetry, the following relations hold:
\begin{equation}
	P_{q_i q_j} = P_{\bar q_i \bar q_j}, \qquad P_{q_i\bar q_j} = P_{\bar q_i q_j}, \qquad P_{q_i g} = P_{\bar q_i g} \equiv P_{qg}/(2 n_f),  \qquad P_{g q_i} = P_{g \bar q_i} \equiv P_{gq}.
\end{equation}

The DGLAP equations can be substantially simplified by moving to a basis in which the majority of equations decouple.
%
The combinations of PDF which decouples are known as \emph{non-singlet}; in particular, since QCD is flavour blind the gluon contribution to the valence distributions\footnote{With a slight abuse of notation, we use the symbol $j$ to identify the PDF $f_j$. }
\begin{equation}
	V_i = q_i - \bar q_i
\end{equation}
and to the differences between quark sea distributions $q^+ = q + \bar q$
\begin{align}
	T_3 = u^+ - d^+ \qquad \qquad 
	T_5 = u^+ + d^+ - 2 s^+ \qquad \qquad
	T_{15} = u^+ + d^+ + s^+ -3 c^+ \nonumber \\
	T_{24} = u^+ + d^+ + s^+ +c^+ - 4b^+ \qquad \qquad
	T_{35} = u^+ + d^+ + s^+ + c^+ + b^+ - 5 t^+
\end{align}
cancel, thereby largely diagonalizing the splitting matrix.
%
The evolution of the $V_i$ and $T_i$ combinations are governed by the splitting functions $P^-$ and $P^+$ respectively, which at LO read
\begin{equation}
	P^{+ (0) } (z) = 	P^{- (0) } (z) = \frac{C_F}{2 \pi} \left(\frac{1+z^2}{1-z} \right)_+.
\end{equation}

The only combination which couples to the gluon is the so-called \emph{singlet} quark PDF $\Sigma = \sum_i q^+_i  =\sum_i (q_i + q_j) $.
%
The evolution of the gluon and singlet PDF is thus controlled by the matrix
\begin{equation}
	\left( \begin{array}{cc}
		P_{gg} & P_{gq} \\
		P_{qg} & P_{qq}
	\end{array} 
	\right).
\end{equation}
At LO, $P^{(0)}_{qq} (z) $ is given by eq.~\eqref{eq:splitting} and 
\begin{align}\label{eq:APsplittingLO}
	P_{gg}^{(0)} (z) &= \frac{C_A}{\pi} \left[ \frac{z}{(1-z)_+} + \frac{1-z}{z} + z (1-z) \right] + \frac{11 C_A-2 n_f}{12 \pi} \delta(1-z), \nonumber \\
	P_{gq}^{(0)} (z) &= \frac{C_F}{2\pi} \left[\frac{1+(1-z)^2}{z} \right] \nonumber \\
	P_{qg}^{(0)} (z) &= \frac{n_f}{2 \pi} \left[ z^2 + (1-z)^2 \right].
\end{align}

It is worth noticing that the convolution structure appearing in eq.~\eqref{eq:AP}, and which we have already encountered in Chapter~\ref{ch-qcd}, has the form of a Mellin convolution
\begin{equation}
(f \otimes g) (x) \equiv \int_x^1 \frac{dz}{z} f(z) g\left( \frac{x}{z} \right),	
\end{equation}
which is symmetric under the change of variable $z \rightarrow x/z$. 
%
The convolution is diagonal under Mellin transform
\begin{equation}
	\mathcal { M } [f] (N) \equiv {\bm f} (N) = \int_0^1 dz \, z^{N-1} f(z),
\end{equation}
such that in Mellin space one has
\begin{equation}
	\mathcal { M } [f \otimes g] (N) = {\bm f} (N) {\bm g} (N).
\end{equation}
By taking the Mellin moments of eq.~\eqref{eq:AP} therefore
\begin{equation}\label{eq:APN-space}
	\mu^2 \frac{\partial}{\partial \mu^2} {\bm f} _j (N, \mu^2) = \gamma_{jk} (N-1,\as(\mu^2)) {\bm f}_k (N, \mu^2) 
\end{equation}
where $\gamma_{ij}$ are known as Altarelli-Parisi anomalous dimensions and we have used the convention (customarily used in small-$x$ physics)
\begin{equation}
	\gamma_{ij} (N, \as)  = \int_0^1 dz \, z^N P_{ij} (z, \as) .
\end{equation}

The universality of the splitting functions --- which appears naturally in the RGE approach --- can be understood by giving a physical interpretation to $P_{ij}$~\cite{Altarelli:1977zs}.
%
By recasting eq.~\eqref{eq:simpleDGLAP} as
\begin{equation}
	q (x, \mu^2) + d q (x, \mu^2) = \int_0^1 dy \int_0^1 dz \delta(zy - x) q (y, \mu^2) \left[\delta (z - 1) + \frac{\alpha(\mu^2) }{2 \pi} P^{(0)}_{qq}(z) d \ln \frac{\mu^2}{\mu_0}\right]
\end{equation}
%where for simplicity we have defined $t= \ln \mu^2$. 
%
where $\mu_0$ is a reference scale. 
%
We can interpret the quantity 
\begin{equation}
	\delta (z - 1) + \frac{\alpha(\mu^2) }{2 \pi} P^{(0)}_{qq}(z) d \ln \frac{\mu^2}{\mu_0^2} = \mathcal P_{qq} 
\end{equation}
as the probability density of finding a quark inside a quark, with a fraction $z$ of the longitudinal momentum of the parent quark and with transverse momentum smaller than $\mu$.
%
We can thus interpret the splitting function as the order $\as$ expression for the variation per unit $\ln \frac{\mu^2}{\mu_0^2}$ of the probability density.
%
Note that since there are $\delta(1-z)$ terms also at order $\as$ --- see eq.~\eqref{eq:splitting} --- the probability for a quark to remain a quark with the same energy is lowered by the interaction. 

Interpreting splitting functions as probabilities allows one to readily compute the splitting functions from the QCD vertices $q \rightarrow q g$, $g \rightarrow q \bar q$, $g \rightarrow gg$. 
%
Typically, one first computes the regular part for $z < 1$ and fixes the $\delta (1-z)$ terms by imposing charge and momentum conservation.
%
The probabilistic interpretation implies that splitting functions are positive definite for $z < 1$.

\subsection{Sum rules}


The behaviour of the splitting functions is further constrained by very general arguments, known as sum rules. 
%
Sum rules are based on the observation that there are some quantities that cannot be modified by DGLAP evolution, as the QCD Lagrangian separately conserves fermion number, flavour and momentum.
%
For instance, though the distribution of the momentum among quarks and gluons may vary, the total momentum shared by partons should be equal to the total momentum of the proton.
%
Similarly, the total barionic number --- computed as the number of quarks minus the number of antiquarks --- cannot change.
%
Therefore, at least asymptotically, we have
\begin{align}
	\int_0^1 dz [\Sigma (z,\mu^2) + g (z,\mu^2) ] & = 1,\\
	\int_0^1 dz [q(z,\mu^2) - \bar q (z,\mu^2) ] &= v_q 
\end{align}
where $v_q = 2, 1, 0 \ldots$ for $u$, $d$, $s$, $\ldots$ quarks. 
%
By considering the Mellin moments of these equations, it is possible to recast these sum rules into constraints on the splitting functions:
\begin{align}
	\int_0^1 dz P_{qq}  (z) = 0, \qquad \int_0^1 dz [ P_{qq}  (z) + P_{gq} (z) ] = 0, \qquad \int_0^1 dz [ P_{qg}  (z) + P_{gg} (z) ] &= 0.
\end{align}
These relations constrain both the qualitative behaviour and the solutions of the evolution equations, and they also simplify the derivation of the splitting function as $P_{qg}$ is now related to $P_{gg}$ and $P_{qq}$. 

\subsection{Solutions of the DGLAP equations}

To obtain a solution of the DGLAP equations one must solve the $2 n_f -1 $ integro-differential equations for the non-singlet contribution and a system of two coupled integro-differential equations for the gluon and the singlet.

There are two main strategies to address this problem.  
%
The most direct approach is to solve the equations in direct space. 
%
This procedure is used in codes such as \texttt{HOPPET}~\cite{Salam:2008qg}, \texttt{QCDNUM}~\cite{Botje:2010ay}, and \texttt{APFEL}~\cite{Bertone:2013vaa}, where the speed of the computation is further improved by resorting to numerical interpolation techniques. 
%
An alternative method, used in codes such as \texttt{QCD-Pegasus}~\cite{Vogt:2004ns}, is to solve the evolution analytically in momentum space, and to obtain the parton densities in $x$-space by computing the inverse Mellin transformation of the evolved $N$-space PDFs
\begin{equation}
	f(x, \mu^2) = \frac{1}{2 \pi i	} \int_{c-i\infty }^{c+i\infty } d N\,  x^{-N} \bm f (N, \mu^2), 
\end{equation} 
where $c$ must be bigger than the rightmost singularity of $\bm f (N, \mu^2)$. 
%
The bottleneck of this approach is the computation of the inversion integral in the complex plane, whose numerical implementation must be particularly efficient. 

In this thesis we will not discuss in details the procedures to solve the DGLAP equations and we refer the reader to the manuals of the aforementioned codes.
%
Some qualitative behaviours of the DGLAP equations can however be understood by looking at the features of the splitting functions eq.~\eqref{eq:APsplittingLO}.
%
For instance, since both $P_{gg}$ and $P_{gq}$ diverge for $z \rightarrow 0$, the quark and gluon PDFs at $x \rightarrow 0$ need to grow at least as fast as $1/x$ at higher scales, since this divergence is introduced by DGLAP evolution independently of the non-perturbative boundary value of the PDFs at $\mu \sim \Lambda_{\rm QCD}$. 
%
Indeed, DGLAP evolution induces partons to lose momentum at higher scales and to shift towards smaller values of $x$, driving a huge growth of the gluon at small $x$.

Whilst perturbative QCD predicts the scale evolution of the parton densities, we still lack a full description of their dependence on $x$.
%
Before addressing the determination of the shape and size of the PDFs, in the next section we will discuss one of the approximation we thus far made by studying the role of quark masses in the factorization framework.  
%
Hitherto, we have worked in massless QCD and we have tacitly assumed that the quarks were massless. 
%
Such an approximation becomes however unjustified whenever the hard scale of the process $Q$ gets closer to the quarks' masses.

\section{Factorization \amper heavy quarks}\label{sec:factheavyquarks}

Quarks are generally classified as `light' or `heavy', although such a distinction has a certain degree of arbitrariness.
%
A convenient definition is based on the relative magnitude of the quark mass and $\Lambda_{\rm QCD}$: quarks whose mass $m \lesssim \Lambda_{\rm QCD} $ are light, whereas quarks whose mass $m \gg \Lambda_{\rm QCD} $ are heavy. 
%
According to such definition, up, down, and strange are light, whereas beauty and top are heavy.
%
The charm quark is usually classified as heavy, though its mass is relatively close to the scale $Q_0$ where non-perturbative behaviour sets in.

As we shall see in section~\ref{sec:pdfdet}, PDF determination relies on the accurate description of several data spanning several order of magnitude.
%
In particular, the hard scale of the process $Q$ can be bigger, comparable or smaller than the mass of one or more heavy quarks. 
%
In this case, the use of a mass-independent scheme such as $\overline{\rm MS}$ is not justified; moreover, precision predictions demand the inclusion of mass corrections when $Q\sim m$.
%
As a consequence, one must resort to so-called variable flavour number schemes (VFNSs), which combine computations performed with a different number of active flavours to obtain a valid theoretical description both close and above the quark mass.


In this section we will start by discussing firstly how such calculations are performed, considering for simplicity the case of three and four active flavours. 
%
We will then discuss and compare different VFNSs which have been proposed for the calculation of DIS structure functions.
%
Finally, we will analyse the special role played by the charm quark. 

\subsection{Massive \amper massless schemes}


The computation of physical quantities, such as cross-sections or structure functions, for a scattering process characterized by a hard scale $Q$ can be performed in different factorization or renormalization schemes.
%
Though the results must be the same to all orders, in general they differ order by order in perturbation theory by higher-order corrections, and acquire in the process a dependence on the renormalization and factorization scales $\mu_R$ and $\mu_F$, typically chosen to be $\sim Q$.
%
The presence of a heavy quark of mass $m_h$ introduces a new scale, dividing the problem into three main regions where different issues are at play:
\begin{itemize}
	\item In the region $Q \ll m_h$ the heavy quark should decouple to avoid unphysical effects at scales much smaller than the heavy quark mass.
	\item In the threshold region $Q \sim m_h$ full dependence on the heavy quark mass is required for precision calculation.
	\item Finally, when $Q \gg m_h$ the partonic cross-sections contain large collinear logarithms of $m_h/Q$, which spoil the accuracy of any fixed-order computation.
\end{itemize}

The description of these three regions requires both suitable renormalization and factorization schemes to ensure manifest decoupling at low scales and the resummation of collinear logarithms at scales much higher than the quark mass, as well as a prescription to include power-suppressed $m_h/Q$ terms relevant for precision phenomenology at $Q \sim m_h $. 
%
We will now briefly summarize the necessary ingredients to construct a scheme (or rather, a sequence of subschemes) to overcome the complications which arise when heavy quarks are involved.
%
For definitiveness, we consider here the case of three massless quarks and one single massive quark.

Let us first notice that from the point of view of renormalization the quark mass does not play an important role; whilst the quark mass acts as an IR regulator, massless-quark loops would still be UV-divergent even if the quark were massive.
%
However, a mass-independent renormalization scheme such as $\overline{\rm MS}$ produces spurious heavy-quark effects at $Q \ll m$ as all flavours participate to $\as$ evolution at any scale. 
%
For this reason, it is appropriate to use the $\overline{\rm MS}$ scheme only for quarks whose mass is lighter than $\mu_R$, whereas it is necessary to use another scheme to ensure the decoupling of heavier quarks. 

Such scheme has been proposed by Collins, Wilczek and Zee in the context of neutral-current processes~\cite{Collins:1978wz}, and was later straightforwardly applied to QCD~\cite{Collins:1998rz}. 
%
The CWZ (or decoupling) scheme is composed by a sequence of subschemes in which the $n_l$ quarks lighter than the renormalization scale $\mu_R$ are renormalized with $\overline{\rm MS}$ terms, whereas UV divergences associated to quarks heavier than the renormalization scale are subtracted at zero external momentum.
%
Since the logarithms of $\mu_R/m_h$ are power suppressed as $\mu_R^2/m_h^2$, the CWZ scheme ensures that at scales $\mu_R \ll m_h$ the graphs containing heavy flavours decouple, whilst the same logarithms are resummed when $\mu_R \gg m_h$.
%
This way, at scales  $\mu_R < m_h$ the running of the strong coupling is identical to the $\overline{\rm MS}$ running, whith $n_f=n_l$.  

The CWZ scheme is effectively a VFNS, as the number of `light' (active, or partonic) and `heavy' (inactive, or non-partonic) flavours depends on the scale and changes in correspondence of the matching scale $\mu_h\sim m_h$.  
%
At the matching scale, the strong couplings in the schemes with three and four active flavours are related by the matching condition
\begin{equation}
	\as^{[3]}(\mu_h) = \as^{[4]} (\mu_h) + \sum_{j=2}^\infty c_j\, \left( \as^{[4]} (\mu_h) \right)^j,  
\end{equation}
whose coefficients $c_j$ can be computed order by order in perturbation theory.
% and are currently known up to four loops~[]. 
%
This relation can be used to relate the coefficients of the perturbative expansion of a generic observable $F( \as)$ in the schemes with three and four active flavours
\begin{equation}
	F( \as) = \sum_k \left(\as^{[3]}\right)^k  F^{[3](k)}  = \sum_k \left(\as^{[4]}\right)^k  F^{[4](k)} 
\end{equation}
by expanding and matching the two expressions order by order once both are written in terms of $\as^{[4]}(\mu_h) $ (or equivalently $\as^{[3]} (\mu_h)$). 

Since the presence of the mass regularizes the collinear divergences, radiative corrections which involve massive quarks are IR finite. 
%
As a consequence, it is possible to factorize only the collinear logarithms associated to massless quarks while retaining the massive collinear logarithms in the partonic cross-sections.
%
This choice, combined with the use of the decoupling scheme for the heavy quarks, leads to the so-called 3 flavour scheme (3FS) or `massive scheme'. 
%
In this scheme, only three quark participate to DGLAP evolution. 
%
By denoting with $\Gamma_{ij}^{[3]}(Q^2)$ the solution of the DGLAP equation with 3 `active' flavours, the PDF thus evolve according to
\begin{equation}
	f_i^{[3]}(Q^2) = \sum_{j, q, \bar q} \Gamma_{ij}^{[3]} (Q^2, Q^2_0) \otimes f_j^{[3]}(Q_0^2).
\end{equation}

A generic structure function in this scheme reads
\begin{equation}\label{eq:3fssf}
	F^{[3]} (Q^2, m_h^2) = \sum_{i=g,q,\bar q, h, \bar h} C_i^{[3]} \left(\frac{m_h^2}{Q^2}, \as^{[3]} (Q^2)  \right) \otimes f_i^{[3]}(Q^2). 
\end{equation}
The coefficient functions are evaluated at fixed order, and thus contain the collinear logarithms due to gluon and light quarks splittings.
%
The effects of the heavy quark mass is retained both in tree-level diagrams and in loop diagrams (e.g. virtual heavy quark loop in gluon propagators, or a gluon splitting into a heavy quark pair).
%
We notice that the sum in eq.~\eqref{eq:3fssf} runs also on $i=h, \bar h$: though only three PDFs participate in DGLAP equation in the 3FS, we allow a contribution from an \emph{intrinsic} heavy quark PDF which could be generated by nonperturbative effects at the scale $Q_0$ below the scale of perturbative heavy quark production.  
%
On the other hand, the heavy quarks appear only through virtual loops and decouple at scales below the production threshold if they were generated perturbatively.

Whereas the 3FS is appropriate for scales $Q \gtrsim m_h$, it becomes problematic at scales $Q \gg m_h$, since the collinear logarithms become increasingly large and spoil the perturbative behaviour of the 3FS result.
%
As a result, when the hard scale is much higher than the quark mass it is opportune to factorize the massive logarithms into the definition of the PDFs, and to resum them with DGLAP evolution, leading to a 4 flavour (or `massless') scheme.
%
The PDFs thus evolve according to
\begin{equation}
	f_i^{[4]}(Q^2) = \sum_{j=g, q, \bar q, h, \bar h} \Gamma_{ij}^{[4]} (Q^2, Q^2_0) \otimes f_j^{[4]}(Q_0^2).
\end{equation}
where $ \Gamma_{ij}^{[4]} $ is the solution of the DGLAP equation with four active flavour, which thus resums also the logarithms generated by heavy quark splittings. 
%
At scales $Q \gg m_h$, the structure functions are readily obtained using standard $\overline{\rm MS}$ counterms for all the active quark, and can be written as 
\begin{equation}\label{eq:4fssf1}
	F^{[4]} (Q^2, m_h^2) = 	F^{[4]} (Q^2, 0) + \mathcal O \left(\frac{m_h^2}{Q^2} \right) =  \sum_{i=g,q,\bar q, h, \bar h} C_i^{[4]} \left(0, \as^{[4]} (Q^2)  \right) \otimes f_i^{[4]}(Q^2) + \mathcal O \left(\frac{m_h^2}{Q^2} \right) . 
\end{equation}
where $C_i^{[4]} \left(0, \as^{[4]} (Q^2)  \right) $ are massless coefficient function and are now finite as the logarithmic divergence has been subtracted.  

The PDFs in the 3FS and in the 4FS are related by the matching conditions 
\begin{equation}\label{eq:pdfmatching}
	f_i^{[4]} (\mu_h^2) = \sum_{j=g, q, \bar q, h, \bar h}  K_{ij} \left( \frac{m_h^2}{Q^2} \right) \otimes f_j^{[3]} (\mu_h^2).
\end{equation}
By inserting this expression into eq.~\eqref{eq:4fssf1} we obtain that 
\begin{equation}\label{eq:masslesslimitcf}
 \sum_{j=g, q, \bar q, h, \bar h} C_i^{[4]} (0)  \otimes   K_{ij} \left( \frac{m_h^2}{Q^2} \right) = C_i^{[3,0]} \left( \frac{m_h^2}{Q^2} \right)
\end{equation}
where $C_i^{[3,0]} $ is the 3FS massive coefficient function with all power-suppressed term set to zero. 
%
The matching condition can therefore be computed simply by calculating DIS structure functions in the 3FS and in the 4FS and expanding order by order in the same $\alpha_s$. 


\subsection{Combining fixed order \amper resummation}

The use of formula~\eqref{eq:4fssf1} above threshold, combined with the use of the 3FS results below threshold, leads to the so-called Zero-Mass (ZM) scheme. 
%
Eq.~\eqref{eq:4fssf1} is appropriate only at scales much higher than the heavy quark mass, but as it neglects all power-suppressed corrections it fails to reproduce the fixed order at the threshold.
%
At that scale mass corrections are important and should be restored, leading to a structure function
\begin{equation}\label{eq:4fssf2}
	F^{[4]} (Q^2, m_h^2)  =  \sum_{i=g,q,\bar q, h, \bar h} \tilde C_i^{[4]} \left(\frac{m_h^2}{Q^2}, \as^{[4]} (Q^2)  \right) \otimes f_i^{[4]}(Q^2)
\end{equation}
which depends on coefficient functions $\tilde C_i^{[4]} \left(m_h^2/Q^2, \as^{[4]} (Q^2)  \right)$, which now include mass effects. 
%
There exist several prescriptions to reinstate the mass corrections, which lead to different formulations of VFNSs\footnote{To distinguish them from the ZM scheme, sometimes these schemes are called General-Mass (GM) schemes.}. 
%
The freedom to incorporate the mass corrections in the 4FS result essentially derives from the assumption that the heavy-quark PDF is perturbatively generated and vanishes at threshold.
%
This is equivalent to imposing a boundary condition on the perturbative evolution, as terms involving the heavy quarks in eq.~\eqref{eq:pdfmatching} can be dropped.
%
As a consequence, various incarnations of VFNSs may differ by subleading terms which are small but nevertheless present at any order in perturbation theory.
%
As we will see in the next section, this ambiguity is not present if the sum in eq.~\eqref{eq:pdfmatching} runs also on the heavy quark.


Let us now briefly summarize the main VFNS currently in use. 
%
For a review and a comparison among these schemes, see e.g. sect. 22 of ref.~\cite{Binoth:2010nha}.

\begin{itemize}
	\item {\scshape ACOT}. The ACOT scheme~\cite{Aivazis:1993pi,Aivazis:1993kh,Collins:1998rz,Tung:2001mv}  is based on a factorization theorem proven to all orders by Collins~\cite{Collins:1998rz} which can be considered as an extension of the massless $\overline {\rm MS}$ scheme to the massive case. 
	%
	The basic idea of this scheme is to retain full mass dependence in the Wilson coefficient; the coefficient functions are obtained by using standard massless collinear counterterms for massless partons, whilst massive collinear counterterms are used for heavy quarks.  
	%
	%By rescaling the heavy-quark Bjorken $x$ to take into account the massive heavy-quark kinematics one obtains a variant of the scheme dubbed ACOT-$\chi$~[].	
	
	\item {\scshape S-ACOT}. Under the assumption that the heavy-quark PDF is generated perturbatively the ACOT scheme can be simplified by moving power corrections between $C_{h,\bar h}^{[4]}$ and  $C_i^{[4]}$ ($i=g,q,\bar q$)  without spoiling the formal accuracy in eq.~\eqref{eq:4fssf2}. 
	%
	This freedom is used to obtain a simplified version of the ACOT scheme in which the heavy quark Wilson coefficients are computed in the massless limit, $\bar C_{h, \bar h}^{[4]} \left(m_h^2/Q^2  \right) = C_{h, \bar h}^{[4]} \left(0 \right) $~\cite{Kramer:2000hn} . 
	%
	By rescaling the heavy-quark Bjorken $x$ to take into account the massive heavy-quark kinematics one obtains a variant of the scheme dubbed S-ACOT-$\chi$~\cite{,Tung:2001mv,Guzzi:2011ew}.	
	%Applying $\chi$-rescaling leads to the S-ACOT-$\chi$ variant~[].
	
	\item {\scshape FONLL}. The original FONLL scheme~\cite{Forte:2010ta,Cacciari:1998it} is based on the observation that to obtain a description of physical quantities valid both at threshold and at high energy it is sufficient to add the 3FS and the 4FS results and to subtract double counting. 
	%
	This way, the FONLL scheme does not require novel factorization schemes as it is based on quantities calculated in well-defined schemes.  
	%
	A phenomenological damping factor is then introduced to (artificially) suppress formally subleading contributions close to threshold.	
	%
	The scheme has been extended to include contributions from initial-state massive quarks in ref~\cite{Ball:2015tna,Ball:2015dpa}. 
	%
	If such contributions are included, the FONLL scheme is formally equivalent to ACOT to all orders in perturbation theory, whereas the original formulation is equivalent to S-ACOT~\cite{Ball:2015dpa}. 
	\item {\scshape TR}. The TR scheme~\cite{Thorne:1997ga} puts the emphasis on the threshold behaviour.  
	% 
	The ambiguity in the definition the massive Wilson coefficient is removed by requiring that physical observables are continuous in the matching region.
	%
	To this end, a formally higher-order, $Q$-independent contribution is added to the massless result above threshold.
	%
	As a consequence, the result differs both from S-ACOT and ACOT by higher-order terms.	
	% 
	The scheme has been explicitly extended at NNLO in ref.~\cite{Thorne:2006qt} (TR' scheme).
	
	\item {\scshape BPT}. Recently, an alternative scheme has been introduced in ref.~\cite{Bonvini:2015pxa} in the context of $b \bar b H$ production using an effective field theory (EFT) approach.
	%
	EFTs are a standard tool to describe processes characterized by separate scales, and are therefore particularly convenient to describe processes with heavy quarks in the initial state. 
	%
	The scheme is formally equivalent to S-ACOT and to the original formulation of FONLL. 
		
\end{itemize}

We observe that another source of difference among the VFNSs is related to the perturbative counting. 
%
For instance, whilst ACOT-like schemes perform the perturbative counting in a standard way by counting the explicit powers of $\as$ in the coefficient functions, in the TR schemes the lowest non-vanishing orders in the 3FS and in the 4FS appear at the same time (i.e. the $\mathcal O(\as^0) $ quark-initiated contribution in the 4FS is combined with the $\mathcal O(\as^1) $ gluon-initiated contribution in the 3FS). 
%
Similarly, the FONLL scheme exists in several incarnation, dubbed FONLL-A, FONLL-B, FONLL-C. 
%
In FONLL-A and FONLL-C the counting is performed as in ACOT schemes, whereas FONLL-B is an intermediate scheme which combines $\mathcal O(\as^2)$ massive contributions with $\mathcal O(\as)$ massless contributions. 
%
The FONLL-B counting is somewhat similar to the perturbative counting used in BPT, where the heavy quark PDF is formally treated as a quantity of order $\as$.


\subsection{The curious case of the charm quark} 

Among the heavy quarks, the charm plays a special role. 
%
On one hand, accurate predictions at scales $Q \gtrsim m_c $ require the inclusion of mass effects as for the other heavy quarks. 
%
On the other hand, however, the value of the charm mass is rather close to the scale where one would expect non-perturbative behaviour to kick in.
%
For this reason, the assumption that the charm is perturbatively generated at threshold may not be accurate, as it is possible that a non-vanishing charm distribution is generated by non-perturbative effects.
%
Various models of non-zero --- `intrinsic' --- charm distributions are present in the literature (for a recent review, see~\cite{Brodsky:2015fna}) and several attempts have been made to obtain an empirical determination~\cite{Aubert:1981ix,Harris:1995jx,Dulat:2013hea,Jimenez-Delgado:2014zga,Ball:2016neh,Hou:2017khm}.

As we discussed in the previous section, the various VFNSs typically assume that the heavy quark PDF is perturbatively generated above threshold.
%
As a consequence, the choice of an adequate VFNS becomes important in the presence of intrinsic heavy quark PDFs.
%
In this section we will focus on the FONLL scheme, and we will discuss how it can be extended to incorporate heavy quark effects. 

In the FONLL scheme, a generic structure function can be constructed as
\begin{equation}
	F_{\rm FONLL}(Q^2, m_h^2) = F^{[4]}(Q^2, 0) +  F^{[3]}(Q^2, m_h^2) - F^{[3,0]}(Q^2, m_h^2) 	
\end{equation}
where the last term which subtracts the double counting is defined in term of the so-called massless limit of the 3FS coefficient functions introduced in eq.~\eqref{eq:masslesslimitcf}:
\begin{equation}
	F^{[3,0]}(Q^2, m_h^2) = \sum_{i=g,q,\bar q, h, \bar h} C_i^{[3,0]} \left(\frac{m_h^2}{Q^2}\right) \otimes f_i^{[3]}(Q^2).
\end{equation}
The result is usually conveniently recast in a formula expressed in terms of the 4FS scheme PDFs. 
%
In its original formulation, the assumption that the heavy quark PDF vanishes at threshold allows one to write
\begin{equation}\label{eq:pdfmatching2}
	f_i^{[3]} (Q^2) = \sum_{j=g, q, \bar q}  \tilde K^{-1}_{ij} \left( \frac{m_h^2}{Q^2} \right) \otimes f_j^{[4]} (Q^2).
\end{equation}
where $\tilde K_{ij}$ is the inverse of the matching matrix defined in~\eqref{eq:pdfmatching} in the subspace of the light partons.
%
In this case, the FONLL result can thus be written as
\begin{align}\label{eq:FONLLzic}
		F_{\rm FONLL}(Q^2, m_h^2)\Big|_{\rm zic} =& \sum_{j=g, q, \bar q}\left\{ \sum_{i=g, q, \bar q} \left[C_i^{[3]} \left( \frac{m_h^2}{Q^2} \right) - C_i^{[3,0]}  \left( \frac{m_h^2}{Q^2} \right)  \right]\otimes  \tilde K^{-1}_{ij}  \left( \frac{m_h^2}{Q^2} \right) + C_j^{[4]} \left(0\right)\right\} \otimes  f_j^{[4]} (Q^2) \nonumber\\
		& +  \sum_{i=h, \bar h} C_i^{[4]} \left(0\right) \otimes  f_j^{[4]} (Q^2).
\end{align}

If the assumption that the heavy quark PDF is perturbatively generated at threshold is no longer valid, one needs to construct the 3FS PDFs using the whole inverse of the matching matrix:
\begin{equation}\label{eq:pdfmatching2}
	f_i^{[3]} (Q^2) = \sum_{j=g, q, \bar q, h, \bar h} K^{-1}_{ij} \left( \frac{m_h^2}{Q^2} \right) \otimes f_j^{[4]} (Q^2).
\end{equation}
and the FONLL result is
\begin{align}
			F_{\rm FONLL}(Q^2, m_h^2) =& \sum_{i,j=g, q, \bar q, h, \bar h} \left[C_i^{[3]} \left( \frac{m_h^2}{Q^2} \right) - C_i^{[3,0]}  \left( \frac{m_h^2}{Q^2} \right)  \right]\otimes  K^{-1}_{ij}  \left( \frac{m_h^2}{Q^2} \right) \otimes  f_j^{[4]} (Q^2) \nonumber\\
		& +  \sum_{i=g, q, \bar q h, \bar h} C_i^{[4]} \left(0\right) \otimes  f_j^{[4]} (Q^2).
\end{align}
However, as $ C_i^{[4]} $ and $C_i^{[3,0]}  $ are related by eq.~\eqref{eq:masslesslimitcf}, the difference term vanishes identically, and the expression is simply
\begin{align}\label{eq:FONLLic}
			F_{\rm FONLL}(Q^2, m_h^2) &= \sum_{i,j=g, q, \bar q, h, \bar h} C_i^{[3]} \left( \frac{m_h^2}{Q^2} \right) \otimes  K^{-1}_{ij}  \left( \frac{m_h^2}{Q^2} \right) \otimes  f_j^{[4]} (Q^2)\nonumber\\
			&\equiv  \sum_{i,j=g, q, \bar q, h, \bar h} C_i^{[4]} \left( \frac{m_h^2}{Q^2} \right)  \otimes  f_j^{[4]} (Q^2)
\end{align}
The coefficient functions $C_i^{[4]} (m_h^2/Q^2)$ can be identified with the coefficient functions defined in the ACOT scheme, since the matching conditions $K^{-1}_{ij}$ subtract order by order the unresummed collinear logarithms such that the convolution with the PDFs has a well-behaved perturbative expansion.

The difference between the result in eq.~\eqref{eq:FONLLic} and the original FONLL formulation~\eqref{eq:FONLLzic} can be cast is in a particular compact form~\cite{Ball:2015dpa}
\begin{equation}\label{eq:deltaFONLL}
	\Delta F_{\rm FONLL}(Q^2, m_h^2) = \sum_{h, \bar h} \left [C_i^{[4]} \left( \frac{m_h^2}{Q^2} \right)-C_i^{[4]} (0)  \right]\otimes\left[f_i^{[4]}- \sum_{k,l=g, q,\bar q} K_{ik}\otimes K_{kl}^{-1}\otimes f_l^{[4]} \right]
\end{equation}
which shows that the missing mass corrections in eq.~\eqref{eq:FONLLzic} are entirely contained in the mass dependence of the 4FS heavy quark-initiated contributions.
%
As $\Delta F_{\rm FONLL}$ becomes zero identically if one sets $C_{h, \bar h}^{[4]} ( m_h^2/Q^2) \rightarrow C_{h, \bar h}^{[4]} (0) $ we can also see explicitly that the original FONLL formulation of ref.~\cite{Forte:2010ta} is equivalent order by order to S-ACOT. 

Eq.~\eqref{eq:deltaFONLL} shows manifestly that $\Delta F_{\rm FONLL}$ is suppressed as  $m_h^2/Q^2$ at $Q^2 \gg m_h^2$.
%
On the other hand, $\Delta F_{\rm FONLL}$ is generally $\mathcal O (1)$ at threshold unless the heavy quark distribution is purely perturbative. 
%
In that case, at the initial scale $Q_0$ the difference term is identically zero as eq.~\eqref{eq:pdfmatching2} can be used, whilst for $Q > Q_0$, and with the matching matrix truncated at order $\as^j$, we can see that
\begin{equation}
	f_i^{[4]}(Q^2) - \sum_{k,l=g, q,\bar q} K_{ik}\otimes K_{kl}^{-1}\otimes f_l^{[4]} (Q^2) \sim \mathcal O \left(\as^{j+1} \ln^{j+1 } \frac{m_h^2}{Q^2}\right),
\end{equation}
and so in absence of intrinsic heavy quark distributions $\Delta F_{\rm FONLL}$ is subleading at $Q\sim m_h$.

Whilst in case of top and beauty it is likely safe to assume that the heavy quark PDF is purely perturbative, it is possible that in presence of intrinsic charm one should in principle compute massive coefficient functions with incoming charm, unless some assumptions are made on the nature of the intrinsic charm density.
%
For instance, if one assumes that the intrinsic contribution is $\mathcal O (\Lambda_{\rm QCD}^2/m_h^2)$ then  $\Delta F_{\rm FONLL}$ is formally suppressed by $\Lambda_{\rm QCD}^2 /Q^2$, and is therefore a higher-twist effect, beyond the accuracy of the factorization theorem. 
%
Recent analyses have suggested that the impact of $\Delta F_{\rm FONLL}$ is indeed small~\cite{Ball:2016neh}, though there is no conclusive evidence on the nature of intrinsic charm. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[thb]
\centering
   \includegraphics[width=0.49\textwidth,page=1]{figures/NLOIC_thesis.pdf}
 \includegraphics[width=0.49\textwidth,page=3]{figures/NLOIC_thesis.pdf}
  \caption{\small The charm structure function $F_2^c$ computed using different heavy quark schemes at NLO accuracy for two different values of $x$, computed with PDFs from ref.~\cite{Ball:2016neh}}
 \label{fig:ACOTvsSACOT}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


From a purely intuitive point of view, however, one could argue that the best accuracy is obtained by VFNSs which respect particle physics kinematics, like the ACOT scheme.
%
Since the calculation of massive coefficient functions is however rather cumbersome (currently, only the $ \mathcal O (\as)$ diagrams with incoming heavy quarks are known~\cite{Hoffmann:1983ah,Kretzer:1998ju}), the accuracy of calculations in the presence of intrinsic PDFs can be improved by restoring the massive kinematics in contributions computed in the massless limit.
%
In fig.~\ref{fig:ACOTvsSACOT}, we compare the charm structure function $F_2^c $ (the part of the structure function in which the struck quark is a charm) at order $\as$, using as input a PDF set where the charm density is fitted to data and therefore can take non-zero values below the matching scale. 
%
We observe that there are some differences at large-$x$ between S-ACOT and ACOT when $Q\sim m_c$, whereas S-ACOT-$\chi$ is always very close to ACOT\footnote{There are several prescriptions for $\chi$-rescaling in the literature. Here we restore the massive kinematics by replacing the integrals of the form $x \int_x^1 dz f(z) C(x/z)$ which appear in the computation of the heavy-quark initiated contribution in the massless scheme with $\chi \int_\chi^1 dz f(z) C(\chi/z)$, where $\chi=x (1+4m_c^2/Q^2)$. With this prescription, S-ACOT-$\chi$ and ACOT coincide at order $\as^{0}$. }. 


\section{Review of PDF determination}\label{sec:pdfdet}

The knowledge of the functional form of parton distribution function is essential for almost any theoretical prediction at hadron colliders.
%
Their determination from first principles, however, requires an understanding of QCD at non-perturbative scales $Q\sim \Lambda_{\rm QCD}$.
%
A possible approach to calculating PDFs is lattice QCD~\cite{Wilson:1974sk}.
%
In lattice QCD the QCD Lagrangian is discretized and the values of quark and gluon fields are considered in a finite-volume lattice.
%
A solution of QCD is then found by sampling the likelihood of different field configurations on the lattice.
%
Lattice QCD has been used successfully in several contexts, such as hadron spectroscopy, $\as$ and CKM determination.
%
However, the accuracy of PDFs based on lattice QCD is not yet competitive with that of PDFs extracted from a fit to experimental data (for a recent review on recent developments in PDF determination from lattice, see~\cite{Lin:2017snn}).

In these analyses, PDFs are parametrized at an initial scale and then evolved to the scale of the data using DGLAP evolution.
%
Theoretical predictions are then built by convoluting the PDFs with hard-scattering cross-sections calculated using perturbative QCD and compared with data.
%
The best fit parameters are finally determined by minimizing an appropriate figure of merit. 

In this section, we first review the main ingredient on PDFs based on global analyses, i.e. the experimental input. 
%
Secondly, we briefly summarize the status of the theoretical calculations for the processes typically included in PDF analysis.
%
We then move to discuss the methodology employed in PDF fits and we summarize possible PDF parametrization and minimization procedures.
%
We finally discuss various strategies for estimating PDF uncertainty.
%
We refer the interested reader to recent reviews on PDF determination~\cite{Roberts:1990ww,Forte:2010dt,DeRoeck:2011na,Perez:2012um,Forte:2013wc,Gao:2017yyd} for a more detailed description of the topics presented here. 


\subsection{Experimental data}\label{sec:expdata}

One of the most important ingredients in the determination of parton densities is the selection of the dataset used in the PDF analysis.
%
The choice is based on the constraining power of the data, which depends on a combination of PDF sensitivity and experimental precision, as well as on the status of the theoretical calculations for the processes examined. 
%
The observables included in PDF fits are typically inclusive enough to guarantee that leading-twist factorization is reliable; for the same reason, the scale of the data included is usually high enough to guarantee that higher-twist contributions are negligible.


Global PDF fits~\cite{Ball:2012cx,Jimenez-Delgado:2014zga,Harland-Lang:2014zoa,Dulat:2015mca,Accardi:2016qay,Alekhin:2017kpj,Ball:2017nwa} include data from a variety of measurements, from fixed-target DIS and Drell-Yan processes, to jet and top-quark production at hadron colliders. 
%
The wealth of available data is shown in Fig.~\ref{fig:kinplot31}, where we show the coverage in the $(x,Q^2)$ plane of a state-of-the-art global analysis.
%
The high-$x$ and low-$Q^2$ region is covered by fixed target experiments, which provided the backbone of the earliest PDF fits.
%
Collider DIS experiments populate the low-$x$ and low- and medium-$Q^2$ region, whereas the high-$Q^2$ region is dominated by recent data from collider experiments at the LHC. 
%
Here we briefly review some of the most relevant processes used in global PDF fits, discussing their PDF sensitivity and the available data, focusing in particular on the processes which are the mainstay of all PDF analyses: deep inelastic scattering and Drell-Yan measurements. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
   \includegraphics[]{figures/aspects0_plot_xq2.pdf}
  \caption{\small Kinematic coverage of a state-of-the art global fit (in this case, ref.~\cite{Ball:2017nwa}) in the $(x,Q^2)$ plane.}
 \label{fig:kinplot31}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{\itshape\mdseries Fixed-target and collider deep inelastic scattering.}

Deep inelastic scattering experiments have been playing a key role in PDF determination since the first semi-quantitative determinations in the early '70s. 
%
In the LO approximation, the neutral current (NC) structure functions $F_2$ and $F_3$ (we recall that at LO $F_2= 2x F_1$) for the process $ep \rightarrow e X$ are given by (see e.g.~\cite{Patrignani:2016xqp})
\begin{align}
	\left[ F_2^\gamma, F_2^{\gamma Z}, F_2^Z\right] &=x \sum_q [e_q^2, 2 e_q g_V^q,(g_V^q)^2 + (g_A^q)^2] (q + \bar q) \\
		\left[ F_3^\gamma, F_3^{\gamma Z}, F_3^Z\right] &=x \sum_q [0, 2 e_q g_A^q,2 g_V^q g_A^q] (q - \bar q) 
\end{align}
where the sums over $q$ run over the active quarks of electric charge $e_q$, $g_A^q = \pm 1/2 $ and $g_V^q = \pm 1/2- 2 e_q \sin^2 \theta_W $, with $\pm$ corresponding to a $u$- or $d$-type quark, respectively.
%
The NC structure functions therefore provide only limited information about flavour separation, and in particular cannot separate quark and antiquarks unless the scale $Q$ is sufficiently high such that the $Z$-mediated contribution becomes important.
%
However, NC DIS on deuterium targets provides a LO handle on the triplet contribution $T^3$ under the assumption of isospin symmetry which relates the quark and antiquark distribution of the proton and the deuteron $u^{(p)}=d^{(n)}$, $u^{(d)}=d^{(p)}$. 

Additional constraint on the quark-antiquark separation is provided by the charged current (CC) processes $e^+ p \rightarrow \bar \nu X$ and $\nu p \rightarrow e^- X$.
%
In the LO approximation and neglecting CKM mixing, the structure functions are (above the charm threshold and below the top threshold)
\begin{align}
	&F_2^{W^-} = 2 x (u + \bar d + \bar s + c ), &F_3^{W^-} = 2 x (u - \bar d - \bar s + c )
\end{align}
whereas the structure functions $F_2^{W^+},\, F_3^{W^+} $ for the processes $e^- p \rightarrow  \nu X$ and $\bar \nu \rightarrow e^+ X$ are obtained by the substitution $c\leftrightarrow s$, $u \leftrightarrow d$. 
%
As a consequence, neutrino data give access to the total valence component $V$.
%
Charm production in neutrino-induced DIS (known as dimuon production) is finally used to probe strangeness, since at LO and neglecting CKM mixing $F_2^{\nu p, c\bar c}=x F_3^{\nu p, c \bar c} = 2 x s$.

Since the gluon does not couple to electroweak final states, the gluon distribution is probed in DIS experiments directly through the small contribution which enters at  $\mathcal O(\as)$, or indirectly via scaling violations encoded in DGLAP evolution. 
%
In principle, $F_L$ measurements could be used to constrain the gluon PDF since $F_L$ is directly sensitive to the gluon PDF~\cite{Altarelli:1978tq}. 
%
The gluon PDF is also constrained by measurements of heavy-quark structure functions obtained in events where charm or bottom mesons are reconstructed in the final state, as the LO contribution (in absence of intrinsic components) is $g\gamma \rightarrow Q \bar Q$. 

There are many available data for DIS measurements, which are delivered either as cross-section or separated in structure functions.  
%
A prominent role is played by the combined NC, CC, charm and beauty structure function measurements at the HERA lepton-proton collider~\cite{Abramowicz:2015mha,H1:2018flt}. 
%
%A non-exhaustive list comprehends NC fixed-target structure functions from EMC~\cite{Aubert:1982tt}, BCDMS~\cite{Benvenuti:1989rh,Benvenuti:1989fm}, NMC~\cite{Arneodo:1996qe,Arneodo:1996kd} (proton and deuteron), SLAC~\cite{Whitlow:1991uw}; CC inclusive structure functions for the scattering of neutrino beams from heavy nuclear target by CHORUS~\cite{Onengut:2005kv} and NuTeV~\cite{Zeller:2001hh} collaborations; dimuon production from NuTeV~\cite{Goncharov:2001qe,Mason:2006qa} and CHORUS~\cite{KayisTopaksu:2008aa}  


\paragraph{\itshape\mdseries Fixed-target and Collider Drell-Yan.}
The so-called Drell-Yan (DY) process --- i.e. the electroweak process in which a quark and antiquark pair annihilate to give a lepton pair --- plays a primary role in PDF analysis due to its constraining power on light flavour decomposition, including strangeness. 
%
At lowest order, and neglecting Cabibbo-suppressed contributions, the partonic subprocesses involved in inclusive EW boson production are
\begin{align}
	\qquad u \bar d, c \bar s \rightarrow W^+, \qquad d \bar u, s \bar c \rightarrow W^-, \qquad  q \bar q \rightarrow \gamma^*/Z
\end{align}
which give access to the flavour composition of the proton since each flavour channel carries a different weight. 
%
Using LO kinematics, the rapidity and the invariant mass of the electroweak boson can be mapped into the values of $x_1$, $x_2$ at which the PDFs are probed:
\begin{equation}\label{eq:DYkin}
	x_{1,2} = \frac{M}{\sqrt{s}}e^{\pm Y},
\end{equation}
where $M$ is the invariant mass of the virtual boson and $Y$ is its rapidity. 
%
Eq.~\eqref{eq:DYkin} therefore relates the PDF sensitivity of DY observables to kinematic variables which can be reconstructed in an experiment (for simplicity, in the following discussion we assume that in the CC case the experimentally inaccessible rapidity of the virtual boson coincide with the measured rapidity of the charged lepton in the final state).

Here we focus on the dominant $u$ and $d$ contributions in a $pp$ collider experiment.
%
Though the presence of a $\bar p$ beam provides additional information on the flavour structure of the proton, the overall constraints are analogue.
%
 In the charged current case, information on the flavour separation can be obtained by considering the ratio of $W^+$ and $W^-$ production differential in rapidity
\begin{equation}
	R_{\pm} = \frac{d \sigma (W^+)/dY}{d \sigma (W^-)/dY}
\end{equation}
and the $W$ asymmetry
\begin{equation}
	A_{W} = \frac{d \sigma (W^+)/dY-d \sigma (W^-)/dY}{d \sigma (W^+)/dY+d \sigma (W^-)/dY}.
\end{equation}
In the central region, where $x_1=x_2=x_0=M/\sqrt{s}$ and one can approximate $\bar u = \bar d$,
\begin{equation}\label{eq:RandA}
	R_{\pm} \simeq \frac{u(x_0)}{d(x_0)}, \qquad A_{W} \simeq \frac{u_V(x_0)-d_V(x_0)}{u_V(x_0)+d_V(x_0)};
\end{equation}
therefore $R_{\pm}$ is sensitive to the ratio between $u$ and $d$, whilst $A_{W}$ is sensitive to the $u$ and $d$ valence difference.
%
Equivalent constraints can be derived in the forward region, see e.g.~\cite{Gao:2017yyd}.

Neutral current DY provides similar information on the $u$ and $d$ content of the proton; there are additional constraints on PDFs at low and intermediate values of $x$ when one moves away from the $Z$ peak and explores the low-invariant mass region.
%
Here the virtual-photon exchange dominates
\begin{equation}
	\frac{d\sigma}{dY} \simeq \sum_q e_q^2 (q (x_1) \bar q(x_2) + q(x_2) \bar q(x_1)),
\end{equation}
and as a consequence the $u \bar u $ channel is enhanced with respect to the $d \bar d$. 
%
This region is also sensitive to the gluon PDF, especially if the cuts on final-state leptons tend to increase the importance of higher-order corrections.
%
Finally, neutral-current Drell-Yan production on fixed deuteron targets can be used to constrain the $\bar u/d$ ratio.
%
In the valence region $x_1 \gtrsim 0.1$, where $q(x_1) \sim q_V(x_1)$, isospin symmetry implies that
\begin{equation}
\frac{\sigma^{pn}}{\sigma^{pp}}	\simeq \frac{\bar d (x_2)}{\bar u (x_2)}.
\end{equation}

%In the previous discussion we have restricted our attention to a $pp$ collider, similar arguments can be made in the case of a $p \bar p$ collider such as Tevatron.

Global PDF analyses use a variety of Drell-Yan measurements, both on fixed target and at hadron colliders. 
%
Among the fixed-target experiments, an important role has been played by the E606 and E866 experiments at Fermilab~\cite{Towell:2001nh}.
%
There is a wealth of collider Drell-Yan measurements, both at the $W$ and $Z$ peak, as well as off peak. 
%
A comprehensive list of recent datasets is presented in ref.~\cite{Gao:2017yyd}.

%Let us mention the recent D0 legacy $W$ asymmetries at Tevatron~\cite{Abazov:2013rja,D0:2014kma}; a comprehensive list of recent datasets from ATLAS, CMS, and LHCb is presented in ref.~\cite{Gao:2017yyd}.

\paragraph{\itshape\mdseries Inclusive jet production.}

Inclusive jet production measurements at hadron colliders have been used since the earliest measurements at Tevatron to constrain the gluon PDF at large $x$.
%
Jet cross sections are experimentally reconstructed using a well-defined jet algorithm; to be compared with theoretical predictions, the jet algorithm used must be IRC safe.
%
The most common choice for data collected at the LHC is the anti-$k_T$ algorithm, though other algorithms are being used. 

The PDF sensitivity of jet production varies according to the definition of the observable and the kinematics.
%
PDF fits typically include single-inclusive jet cross-section data, which are double-differential in jet $p_T$ and rapidity $Y$. 
%
For each event, all jets are considered and included in the same distribution. 
%
The gluon-induced contribution in these measurements dominates at low $p_T$ but is also quite significant at high $p_T$. 
%
Since the quark content of the proton is already rather constrained by DIS and DY measurements, jet data help to handle the gluon PDF in the region of medium and large $x$. 
%
There are several double-differential single-inclusive datasets which can be included in PDF fits; again, we refer to ref.~\cite{Gao:2017yyd} for a comprehensive list.

\paragraph{\itshape\mdseries Transverse momentum of $Z$ bosons.}

Very precise measurements of the inclusive transverse momentum of the $Z$ boson have recently been released by the ATLAS, CMS and LHCb collaborations.
%
The dominant contribution in the region of moderate and large transverse momentum is gluon and quark scattering; as a consequence, the inclusion of $Z$ transverse momentum data can provide additional constraints to the gluon in the medium-$x$ region, which is only partly probed by collider DIS data and jets data. 

\paragraph{\itshape\mdseries Top quark production.}

Another process which provides strong constraints on the gluon PDF, especially at large $x$, is top quark production.
%
At values of $\sqrt{s}$ probed at the LHC the gluon contribution to the top-pair cross-section exceeds 80\%. 
%
Experimental measurements are presented both at the total cross section level at Tevatron, and both at the inclusive and differential level at the LHC. 


\paragraph{\itshape\mdseries Other processes.}

There are other processes which can provide additional constraints on several combinations of PDF, which however we do not have time to discuss in detail.
%
The large-$x$ gluon can be probed also by prompt-photon production, whose dominant contribution is the QCD Compton scattering $qg \rightarrow q \gamma$.
%
$W^\pm+c$ production allows one to put constraint on the strangeness and on the strangeness asymmetry in the proton, whilst single-top production gives an handle on the $b$ quark content of the proton. 
%
Finally, the small-$x$ gluon can be further constrained by including in PDF fits charmed-meson production at hadron colliders, as the dominant channel for this process is $gg\rightarrow c\bar c$.
%
LHCb data~\cite{Aaij:2013mga,Aaij:2015bpa,Aaij:2015bpa} provide information on the gluon PDF down to very small values of $x\sim10^{-6}$, a region which is also important for neutrino astrophysics~\cite{CooperSarkar:2011pa,Gauld:2015yia,Gauld:2015kvh,Garzelli:2016xmx,Gauld:2016kpd}.

\subsection{Theoretical accuracy}

Since parton densities are based on a combination of experimental data and perturbative QCD calculations, the perturbative accuracy of a PDF fit depends on that of the theoretical predictions used in the analysis, that is the splitting functions eq.~\eqref{eq:AP} and the partonic cross-sections which are convoluted with the PDFs. 

PDFs are typically extracted using fixed-order perturbation theory.
%
For most of the processes we have reviewed in section~\ref{sec:expdata} the coefficient functions have been computed to NNLO accuracy, and in some cases up to N$^3$LO.
%
In particular, DIS production is known up to N$^3$LO accuracy in the massless limit~\cite{Moch:2004xu,Vermaseren:2005qc} and to NNLO including mass effects~\cite{Laenen:1992zk,Laenen:1992xs}, and the coefficient functions are implemented in a number of public codes such as \texttt{APFEL}~\cite{Bertone:2013vaa}, \texttt{QCDNUM}~\cite{Botje:2010ay} and \texttt{OpenQCDrad}~\cite{Alekhin:2010sv}. 
%
The NNLO calculation for differential $W$ and $Z$ rapidity distributions in Drell-Yan production has been known since quite some time~\cite{Anastasiou:2003ds,Anastasiou:2003yy,Melnikov:2006di,Melnikov:2006kv}, and there exists several tools to produce theoretical predictions.
%, such as \texttt{FEWZ}~\cite{Gavin:2010az,Gavin:2012sy}, \texttt{DYNNLO}~\cite{Catani:2009sm}, and \texttt{MCFM}~\cite{Campbell:2011bn,Boughezal:2016wmq}. 
%
Single-inclusive jet and inclusive dijet production have been computed up to NNLO accuracy~\cite{Currie:2016bfm,Currie:2017eqf}, and Z $p_T$ distributions have been recently been computed at NNLO by two independent groups~\cite{Boughezal:2015ded,Gehrmann-DeRidder:2016jns,Ridder:2016nkl,Boughezal:2016isb}.
%
The NNLO correction to the total cross-section for top production has been known for a few years, whereas only recently the full NNLO corrections for a variety of differential distribution have become available~\cite{Czakon:2014xsa,Czakon:2015owf,Czakon:2016dgf}.
%
Let us notice that, at this level of accuracy, electroweak (EW) corrections start to be relevant as $\alpha_{\rm EW}\sim \frac{1}{100}\sim \as^2$. 
%
EW corrections are not systematically included in current PDF analysis yet.
%
We refer the reader to ref.~\cite{Gao:2017yyd} for a thorough review of the status of the theoretical calculations for the various processes included in global analysis as well as for a discussion about the current status of EW corrections. 

By convoluting partonic cross-sections computed at NNLO accuracy with DGLAP evolution computed using NNLO splitting functions PDFs can now be determined up to NNLO accuracy. 
%
NLO PDFs are widely used in conjunction with automatic NLO codes to produce NLO-accurate predictions for a variety of processes, whilst optimized LO PDFs are delivered to be used with Monte Carlo event generators~\cite{Sherstnev:2007nd}. 

For the majority of processes included in PDF analysis, fixed order theory accurately describes the data.
%
However, as we will discuss in the Chapter~\ref{ch-res}, in some cases logarithmic-enhanced terms appear at all orders and spoil the perturbative convergence of the series.
%
When this happens, one must supplement the fixed-order description with the resummation of the enhanced terms to all-orders. 
%
We will discuss PDF sets extracted using resummed calculations in Chapter~\ref{ch-respdfs}.


\subsection{PDF Parametrization}

The determination of a set of functions from a finite ensemble of experimental data point is a well-known mathematically ill-posed problem, as there is no unique solution. 
%
As a consequence, though the PDF parametrization should be as general as possible to avoid artificial bias, it is necessary to adopt an {\it ansatz} to obtain a concrete solution.
%
The PDFs are usually parametrized at the initial scale $Q_0 \sim 1-2$ GeV as
\begin{equation}\label{eq:PDFpar}
	x f_i(x,Q_0^2) = x^{\alpha_i} (1-x)^{\beta_i} \mathscr F_i (x, \{ \gamma_i \})  
\end{equation}
where $\mathscr F_i$ is a smooth function and the parameters $\alpha_i, \,  \beta_i$ and $\{\gamma_i \}$ are determined by the fit. 
%
This choice is motivated by the theoretical, non-perturbative expectation that PDFs should behave as a power law at asymptotic values of $x$ (see e.g.~\cite{Ball:2016spl}).
%
In particular, the power behaviour at $x\rightarrow 0$ is predicted by Regge theory~\cite{Regge:1959mz}, whereas the behaviour at $x\rightarrow 0$ is constrained by quark counting rules~\cite{Brodsky:1973kr,Devenish:2004pb,Roberts:1990ww,Devenish:2004pb}.

The parameterization eq.~\eqref{eq:PDFpar} is adopted for all the PDFs entering in the fit (or, typically, for the gluon and a convenient linear combination of the quark PDFs).   
%
In principle, the number of independent fitted PDFs should be equal to thirteen.
%
However, since heavy-quark PDFs are usually assumed to be generated by gluon splitting, it is customary to include seven independent PDFs in the fits (in recent fits by the NNPDF collaboration, the charm PDF is added alongside the other PDFs within the assumption that $c(x,Q_0^2)=\bar c(x,Q_0^2)$, thus the number of fitted PDFs is eight).

The form of $\mathscr F_i$ must be determined from the fit, with the only assumption that it tends to a constant in the limits $x\rightarrow 0$, $x \rightarrow 1$.
%
The specific choice for the interpolation function $\mathscr F_i$ is not uniquely defined and varies between different groups.
%
The simplest option, which has been largely used in the literature, is to assume a polynomial or an exponential polynomial of $x$ or $\sqrt{x}$.
%
As the number of data points increases, however, the need for a more flexible and unbiased parameterization has emerged. 

In recent fits by the MMHT collaboration and the CT10 collaboration the function $\mathscr F_i$ is expanded on a basis of Chebyshev and Bernestein polynomials, respectively.
%
This choice allows one to increase the number of free parameters avoiding large cancellations among terms which plague fits with simpler functional forms, and at the same time reduces the correlations among terms.

The NNPDF collaboration has adopted a somewhat different approach.
%
The functional dependence on $x$ is parametrized by neural networks, which allows for great flexibility and lack of bias due to their redundancy~\cite{DelDebbio:2007ee,Hartland:2018}. 
%
Specifically, NNPDF uses multilayer feed-forward neural networks, whose architecture is fixed for all the PDFs entering in the fit. 
%
The number of free parameters is about one order of magnitude higher with respect to other PDF collaborations; in its latest fit, each PDF has 37 free parameters, and the total number of parameters to be determined is thus 296. 

The rather different number of free parameters to be determined has important consequences on the minimization strategies used by each collaboration.
%
For instance, if the number of parameters becomes too large, the absolute minimum of the figure of merit used to determined the fit quality might not correspond to the best fit as one might start to fit the noise rather than the underlying law.
%
We will discuss the choice of an appropriate figure of merit and various strategies for minimization in the next section.

\subsection{Fit quality \amper strategies for minimization}

The figure of merit used to measure the fit quality is typically the log-likelihood function $\chi^2$
\begin{equation}\label{eq:chi2form1}
	\chi^2 (\{ \zeta_i\} ) = \sum_{i,j}^{N_{\rm dat }} (D_i - T_i(\{ \zeta_i\})) ({\rm cov}^{-1} )_{ij} (D_j - T_j(\{\zeta_i\})),
\end{equation}
where $D_i$ are the data points, $T_i$ are the theoretical predictions expressed in terms of the PDF parameters $\zeta_i$, and the experimental covariance matrix ${\rm cov}$ and its inverse ${\rm cov}^{-1}$ are defined by 
\begin{align}
	({\rm cov})_{ij} &= (\sigma^{\rm uncorr}_{i})^2 \delta_{ij} + \sum_{\kappa=1}^{N_{\rm corr}} \sigma^{\rm corr}_{\kappa, i } \sigma^{\rm corr}_{\kappa, j },\\
	({\rm cov}^{-1})_{ij} &= \frac{\delta_{ij}}{(\sigma^{\rm uncorr}_{i})^2} - \sum_{\kappa,\lambda=1}^{N_{\rm corr}}  \frac{\sigma^{\rm corr}_{\kappa, i }}{(\sigma^{\rm uncorr}_{i})^2} A^{-1}_{\kappa \lambda}  \frac{\sigma^{\rm corr}_{\lambda, j }}{(\sigma^{\rm uncorr}_{j})^2}, & A_{\kappa \lambda} = \delta_{\kappa \lambda} + \sum_{i}^{N_{\rm dat }} \frac{\sigma^{\rm corr}_{\kappa, i } \sigma^{\rm corr}_{ \lambda,i } }{\sigma^{\rm uncorr}_{i}}.
\end{align}
Here $i=1, \ldots N_{\rm dat}  $ indicates the individual data points, affected by uncorrelated uncertainty $\sigma^{\rm uncorr}_{i}$ and $\kappa=1, \ldots {N_{\rm corr}}$ sources of correlated uncertainty $\sigma^{\rm corr}_{\kappa, i } $.
%
In the absence of correlated uncertainties the covariance matrix has non-zero entries only in the diagonal; however, a faithful figure of merit must include information on the correlations, since otherwise the uncertainty might be misestimated. 

The $\chi^2$ eq.~\eqref{eq:chi2form1} is sometimes written in terms of the nuisance parameters $r_\kappa$ as
\begin{equation}\label{eq:chi2form2}
	\chi^2 (\{\zeta_i\}, \{ r_\kappa \}) = \sum_{i=1}^{N_{\rm dat}}\left( \frac{\hat D_i - T_i (\{ \zeta_i\})}{(\sigma^{\rm uncorr}_{i})^2}\right)^2 + \sum_{\kappa=1}^{N_{\rm corr}} r_k^2
\end{equation}
where 
\begin{equation}\label{eq:sysshift}
	\hat D_i  = D_i -  \sum_{\kappa=1}^{N_{\rm corr}} r_\kappa \sigma^{\rm corr}_{\kappa, i } .
\end{equation}
Minimizing eq~\eqref{eq:chi2form2} by assuming purely Gaussian errors with respect to the nuisance parameters one finds
\begin{align}
\tilde r_\kappa = \sum_{i=1}^{N_{\rm dat}}\frac{D_i - T_i}{(\sigma^{\rm uncorr}_{i})^2} \sum_\lambda^{N_{\rm corr}} A_{\kappa \lambda}^{-1} \sigma^{\rm corr}_{\kappa, i },
\end{align}
which can be substituted in eq~\eqref{eq:chi2form2} to give back eq.~\eqref{eq:chi2form1}.  
%
Whilst formally equivalent to eq~\eqref{eq:chi2form2} when $\{r_\kappa \}=\{\tilde r_\kappa \}$, the form~\eqref{eq:chi2form2} can be convenient to study the behaviour of the shifts at the minimum to check their gaussianity.
%
Moreover, figures which compare the data points shifted as in eq.~\eqref{eq:sysshift} to the theoretical predictions allow one to visualize the effect of the correlated uncertainties more effectively~\cite{Pumplin:2002vw}. 

Let us mention that there is a subtleness when multiplicative uncertainties (i.e. such that the size of the uncertainty is proportional to the measured value) are present in the definition of the $\chi^2$.
%
In this case, it has been shown that a $\chi^2$ defined as in \eqref{eq:chi2form1} leads to the so-called {\it d'Agostini bias}~\cite{DAgostini:1993arp}, as the data points subject to downward fluctuations have a smaller normalization uncertainty. 
%
As a consequence, if \eqref{eq:chi2form1} is used the fit tends to systematically undershoot the data.
%
Several solutions have been proposed in the literature.
%
For instance, the NNPDF collaboration uses the so-called $t_0$ definition of the covariance matrix~\cite{Ball:2009qv}: the covariance matrix is constructed by rescaling the multiplicative error by the theory predictions obtained from a previous iteration of the $\chi^2$ minimization.

Once a suitable figure of merit has been constructed, the next step is to find the global minimum in the parameter space spanned by the PDF parameters $\{ \zeta_i\}$.
%
The strategy to find the minimum varies among different groups.
%
If the number of free parameters is moderate, the methods used are typically gradient-based. 
%
Variants of these methods are employed in MMHT and CT analyses, where the Levenberg-Marquardt method~\cite{Levenberg,Marquardt} and the variable metric method provided by the \texttt{MINUIT} package~\cite{James:1975dr} are used, respectively. 

However, the computation of the gradient becomes computationally very challenging if the number of parameters is too large as in the case of NNPDF analyses. 
%
As a consequence, NNPDF follows a gradient-free minimization approach such as the Nodal Genetic Algorithm (NGA)~\cite{Montana:1989}.
%
The strategy of the algorithm is very simple: at each iteration of the minimization procedure, the parameters are varied gaussianly around the search centre and the best-fit parameters are selected for the next iteration.
%
Some care is needed to avoid over-learning, since the algorithm selects only the best candidates at each iteration and is therefore quite sensitive to noise. 
% 
Recent studies based on the NNPDF framework~\cite{Bertone:2017tyb,Carrazza:2017udv} have explored another strategy --- the Covariance Matrix Adaption - Evolutionary Strategy (CMA-ES) --- which is commonly used when gradient descent methods are difficult to apply~\cite{,Hansen2001ecj,Hansen16a} . 

\subsection{Error propagation: Hessian  \amper  Monte Carlo approaches}

Until the late '90s, PDF uncertainty could be assessed only by comparing predictions obtained using different PDF sets. 
%
When PDF started to be a tool for precision physics, a reliable estimate of the uncertainty related to PDF became mandatory. 
%
Current PDF sets are thus always delivered with an associated PDF uncertainty.
%
In this section we will summarize two of the most common methods to evaluate PDF error: the Hessian method and the Monte Carlo method.
%
Another method of error propagation, the Lagrange multiplier method, is reviewed in refs.~\cite{DeRoeck:2011na,Hartland:2014nha,Gao:2017yyd,}.

\paragraph{\itshape\mdseries Hessian method.} The Hessian method is the most common method of uncertainty determination in PDF fitting. 
%
Qualitatively, the method is based on studying the perturbations of the $\chi^2$ around its minimum when the fitting parameters $\{\zeta_i \}$ are varied; the uncertainty on the physical observables is then determined geometrically by considering the values computed using the perturbed parameters. 

Let us discuss the method more quantitatively. 
%
Close to its minimum $\tilde \chi^2$, the variations of the $\chi^2$ can be  approximated as quadratic
\begin{equation}
	\Delta \chi^2 \equiv \chi^2 - \tilde \chi^2 = \sum_{i,j}^{N_{\rm par}} (\zeta_i - \tilde\zeta_i ) H_{ij} (\zeta_j - \tilde\zeta_j ),
	\end{equation}
where $\{ \tilde\zeta_i \} $ correspond to the best-fit parameters and we have defined the Hessian matrix
\begin{equation}\label{eq:hessianlinear}
	H_{ij} \equiv \frac{1}{2} \frac{\partial^2 \chi^2}{\partial \zeta_i \partial \zeta_j } \Bigg|_{\{  \zeta_i\} = \{ \tilde \zeta_i\}}.
\end{equation}
In principle, the error on a generic observable $\mathcal F$ which depends on the PDFs could be determined by simple linear error propagation as
\begin{equation}
	\sigma_{\mathcal F} = T \left( \sum_{i,j}^{N_{\rm par}} \frac{\partial \mathcal F}{\partial \zeta_i} (H)^{-1}_{ij}  \frac{\partial \mathcal F}{\partial \zeta_i} \right)^{1/2}
\end{equation}
where $T=\sqrt{\Delta \chi^2}$ is the so-called tolerance factor, which allows one to match the range of variation of the fit parameters to the confidence interval associated to the PDF uncertainties. 

However, eq.~\eqref{eq:hessianlinear} presents some limitations since the partial derivatives of the observables with respect to the fit parameters are generally unknown.
%
Moreover, numerically instabilities may arise due to very different variations of the $\chi^2$ in different directions in parameter space~\cite{DeRoeck:2011na}. 
%
One can overcome these limitation simply by diagonalizing the hessian matrix~\cite{Pumplin:2000vx,Pumplin:2001ct}.
%
After the diagonalization procedure, the error on an observable $\mathcal F$ is given by 
\begin{equation}
	\sigma_{\mathcal F}^2 = \frac{1}{2} \left( \sum_{i}^{N_{\rm par}} \left[ \mathcal F(S^+_i) - \mathcal F(S^-_i)  \right] \right)^{2},
\end{equation}
where $S^\pm$ are PDF set constructed along the eigenvector directions, displaced by the desired $\Delta \chi^2$.  

The uncertainties in the Hessian procedure depend somewhat on the choice of the value of the tolerance $T$. 
% 
For specialized PDF sets based on a restricted dataset one may use the textbook tolerance $\Delta \chi^2 = 1$, although the final uncertainty may be larger if methodological uncertainties are taken into account e.g. by considering variations of the parametrization as in the HERA PDF family~\cite{Abramowicz:2015mha}. 
%
However, in the context of global PDF fits the value of the tolerance is typically higher to take into account experimental inconsistencies or methodological uncertainties.
%
For this reason, CT and MMHT collaborations use a larger value for the tolerance, which in recent fits by the MMHT collaboration is determined dynamically.


\paragraph{\itshape\mdseries The Monte Carlo method.} 

The Monte Carlo (MC) method is a complementary method for determination of the PDF uncertainty, which is based on a MC procedure in the space of the experimental data. 
%
The method is designed to construct a faithful representation of the uncertainties present in the initial data without any assumption on their nature.

The first step in the MC method is the construction of an ensemble of $N_{\rm rep}$ of artificial data replicas (dubbed {\it pseudodata} replicas) for every data point included in the fit, generated according to the probability distribution of the initial data. 
%
For a given experimental measurement of a generic observable $\mathcal F^{\rm exp}$, characterized by a total uncorrelated uncertainty $\sigma^{\rm uncorr}$, $\kappa = 1, \ldots N_{\rm corr}$ correlated uncertainties $\sigma^{\rm corr}_\kappa$ the artificial MC replicas $\mathcal F^{{\rm art},k}$ are constructed as~\cite{Forte:2002fg}
\begin{equation}
	\mathcal F^{{\rm art},\ell}  = \mathcal N^\ell \mathcal F^{{\rm art},\ell}  \left( 1 + \sum_{\kappa = 1}^{N_{\rm corr}} r^{(\ell)}_\kappa \sigma^{\rm uncorr}_\kappa + r^{(\ell)} \sigma^{\rm uncorr}  \right) , \qquad \ell = 1, \ldots N_{\rm rep},
\end{equation}
where $r$ are independent random gaussian numbers and the normalization of the probability distribution is determined by the normalization pre-factor $\mathcal N^\ell$.
%
Several analysis have shown that a faithful representation of the data and their correlations requires $\sim 1000 \, N_{\rm rep}$. 

Once a MC sample of the experimental data is available, one fit is performed for each pseudodata replica.
%
At the end of the procedure therefore there exist $N_{\rm rep}$ equally probable PDF sets which reliably describe the probability density of parton densities in PDF space based on the original experimental errors.
%
The central values and uncertainties of an observable $\mathcal F$ are finally obtained as the average and the variance over the replica ensemble
\begin{align}
	\langle \mathcal F \rangle &= \frac{1}{N_{\rm rep}} \sum_{\ell=1}^{N_{\rm rep}} \mathcal F^\ell\\ 
	\sigma^2_{\mathcal F} &= \frac{1}{N_{\rm rep}-1} \sum_{\ell=1}^{N_{\rm rep}} (\mathcal F^\ell- \langle \mathcal F^{\ell} \rangle)^2
\end{align}
where $\mathcal F^{\ell}$ denotes the value of the observable $\mathcal F$ evaluated with the PDF replica $\ell$. 
%
Since the MC method naturally propagates the experimental error without any assumption, there is no need to increase the tolerance.
%
In case of fully-consistent datasets, the MC method and the Hessian method with $\Delta \chi^2=1$ coincide~\cite{Dittmar:2009ii}.
%
Algorithms to construct a MC representation of a Hessian set~\cite{Watt:2012tq} and, conversely, a Hessian representation of a MC set~\cite{Carrazza:2015aoa} are available.


\noindent \paragraph{\itshape\mdseries} Let us finally notice that what is commonly referred as ``PDF uncertainty'' currently includes the experimental uncertainty on the data used to extract the PDF (and possibly other methodological uncertainties), but does not include any theory error.
%
For instance, since PDFs are extracted using fixed-order QCD, one should take into account the uncertainty due to missing higher orders.
%
The theory error has been always assumed to be negligible with respect to the experimental and methodological uncertainty.
%
Due to the wealth of very precise data and the constant methodological improvements, however, the theory error is now comparable to the PDF uncertainty in a wide range of $x$ and $Q^2$, and will eventually become dominant.
%
Whereas a thorough study of theory errors in PDF determination is still waited for, preliminary studies of theoretical uncertainties in PDF analyses have been presented in~\cite{Bendavid:2018nar}. 



==> text/preface.tex <==
\chapter*{\label{ch:preface}Preface}
\addcontentsline{toc}{chapter}{Preface} 



This document introduction won't serve as a complete primer on \LaTeX.  There are plenty of those online, and googling your questions will often get you answers, especially from \url{http://tex.stackexchange.com}.

Instead, let's talk a little about a few of the features and packages lumped into this template situation.  The \verb|savequote| environment at the beginning of chapters can add some wittiness to your thesis.  If you don't like the quotes, just remove that block.

For when it comes time to do corrections, there are two useful commands here.  First, the \verb|mccorrect| command allows you to highlight a short correction \mccorrect{like this one}.  When the thesis is typeset normally, the correction will just appear as part of the text.  However, when you declare \verb|\correctionstrue| in the main \verb|Oxford_Thesis.tex| file, that correction will be highlighted in blue.  That might be useful for submitting a post-viva, corrected copy to your examiners so they can quickly verify you've completed the task.

\begin{mccorrection}
For larger chunks, like this paragraph or indeed entire figures, you can use the \verb|mccorrection| environment.  This environment highlights paragraph-sized and larger blocks with the same blue colour.
\end{mccorrection}

Read through the \verb|Oxford_Thesis.tex| file to see the various options for one- and two-sided printing, including or excluding the separate abstract page, and turning corrections and draft footer on or off, and the separate option to centre your text on the page (for PDF submission) or offset it (for binding).  There is also a separate option for master's degree submissions, which changes identifying information to candidate number and includes a word count.  (Unfortunately, \LaTeX has a hard time doing word counts automatically, so you'll have to enter the count manually if you require this.)


